Specular: Towards Secure, Trust-minimized Optimistic Blockchain Execution

An optimistic rollup (ORU) scales a blockchain's throughput by delegating computation to an untrusted remote chain (L2), refereeing any state claim disagreements between mutually distrusting L2 operators via an interactive dispute resolution protocol. State-of-the-art ORUs employ a monolithic dispute resolution protocol that tightly couples an L1 referee with a specific L2 client binary--oblivious to the system's higher-level semantics. We argue that this approach (1) magnifies monoculture failure risk, by precluding trust-minimized and permissionless participation using operator-chosen client software; (2) leads to an unnecessarily large and difficult-to-audit TCB; and, (3) suffers from a frequently-triggered, yet opaque upgrade process--both further increasing auditing overhead, and broadening the governance attack surface. To address these concerns, we outline a methodology for designing a secure and resilient ORU with a minimal TCB, by facilitating opportunistic 1-of-N-version programming. Due to its unique challenges and opportunities, we ground this work concretely in the context of the Ethereum ecosystem--where ORUs have gained significant traction. Specifically, we design a semantically-aware proof system, natively targeting the EVM and its instruction set. We present an implementation in a new ORU, Specular, that opportunistically leverages Ethereum's existing client diversity with minimal source modification, demonstrating our approach's feasibility.

==> text/opcodes-table.tex <==
\newcommand{\stateP}{\texttt{state}\xspace}
\newcommand{\opcodeP}{\texttt{opcode}\xspace}
\newcommand{\dataP}{\texttt{L1-data}\xspace}
\newcommand{\execerrorP}{\texttt{exception}\xspace}
\newcommand{\stackP}{\texttt{stack}\xspace}
\newcommand{\memReadP}{\texttt{memory-R}\xspace}
\newcommand{\memWriteP}{\texttt{memory-W}\xspace}
\newcommand{\accReadP}{\texttt{account-R}\xspace}
\newcommand{\accWriteP}{\texttt{account-W}\xspace}
\newcommand{\storageReadP}{\texttt{storage-R}\xspace}
\newcommand{\storageWriteP}{\texttt{storage-W}\xspace}
\newcommand{\codeP}{\texttt{code}\xspace}
\newcommand{\logP}{\texttt{log}\xspace}

\begin{table*}[t]
  % \begin{adjustwidth}{-.5in}{-.5in}
  \centering \resizebox{\textwidth}{!}{\small
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{\textbf{Opcodes}} & 
    \multicolumn{8}{c|}{\textbf{Proof types}} \\
    \cline{2-9}
    % \cmidrule{2-9} \vspace{-1em} \\
     & \stackP &  \memReadP &  \memWriteP &  \accReadP &  \accWriteP &  \storageReadP &  \storageWriteP & \codeP \\
    
    % \hline
    % \texttt{JUMPDEST} & & & & & & & & \\
    
    \hline
    \makecell{\texttt{MLOAD, KECCAK256,} \\ \texttt{ CALLDATALOAD}} & 
    \checkmark & \checkmark & & & & & & \\
    
    \hline
    \texttt{MSTORE, MSTORE8} & 
    \checkmark & & \checkmark & & & & & \\
    
    \hline
    \makecell{\texttt{CALLDATACOPY,} \\ \texttt{RETURNDATACOPY}} & 
    \checkmark & \checkmark & \checkmark & & & & & \\
    
    \hline
    \texttt{BALANCE, SELFBALANCE} & 
    \checkmark & & & \checkmark & & & & \\
    
    \hline
    \texttt{SLOAD} & 
    \checkmark & & & \checkmark & & \checkmark & & \\
    
    \hline
    \texttt{SSTORE} & 
    \checkmark & & & & \checkmark & & \checkmark & \\
    
    \hline
    \texttt{CODESIZE} & 
    \checkmark & & & & & & & \checkmark \\
    
    \hline
    \texttt{CODECOPY} & 
    \checkmark & & \checkmark & & & & & \checkmark \\
    
    \hline
    \texttt{EXTCODESIZE, EXTCODECOPY} & 
    \checkmark & & \checkmark & \checkmark & & & & \checkmark \\
    
    \hline
    \texttt{EXTCODEHASH} & 
    \checkmark & & & \checkmark & & & & \\
    
    \hline
    \makecell{\texttt{RETURN, REVERT,} \\ \texttt{STOP, INVALID}} & 
    \checkmark & \checkmark & & & \checkmark & & & \\
    
    \hline
    \makecell{\texttt{CREATE, CREATE2,} \\ \texttt{CALL, CALLCODE,} \\ \texttt{DELEGATECALL, STATICCALL,} \\ \texttt{SELFDESTRUCT}} & 
    \checkmark & \checkmark & & \checkmark & \checkmark & & & \\
    
    \hline
    \texttt{LOG0$\sim$LOG4} & \checkmark & \checkmark & & & & & & \\
    
    \hline
    All others (e.g. arithmetic ops) & 
    \checkmark & & & & & & & \\
    
    \hline
  \end{tabular}}
  % \end{adjustwidth}
%   \vspace{1em}
  \caption{
      \textbf{One-step proof composition for each EVM opcode.} The required proofs depend on which data structures are accessed by the instruction.
      In addition to the above proof types, \stateP, \opcodeP, and \dataP are included for all opcodes.
      Some opcodes require multiple proofs of the same type---for example, \texttt{RETURN}, \texttt{REVERT}, \texttt{STOP}, and \texttt{INVALID} require an additional \stateP proof for the OSS of the last execution step.
      Some opcodes require special types of proofs not listed in the table, as discussed in \Cref{sec:other_proof}.
      % \ujval{not sure if this is the right place for this}
      \todolowprio{consider using num of proofs instead of \checkmark}
      Note: "read" and "write" suffixes are abbreviated as \texttt{R} and \texttt{W} respectively.
  }
  \label{table:opcodes}
\end{table*}

==> text/scratch.tex <==
\ujval{scratchwork}

